Toward Quantum Utility in Correlated Topological Matter: Variational Preparation of Fractional Quantum Hall Manifolds

We investigate the use of variational quantum algorithms to prepare and characterize fractional quantum Hall states on near-term quantum processors. Focusing on the $\nu=1/3$ Laughlin phase described by the $V_1$ Haldane pseudopotential, we formulate the lowest-Landau-level problem in second quantization, and implement particle-number-preserving variational circuits combined with the variational quantum eigensolver (VQE) and variational quantum deflation (VQD). We benchmark the approach in two complementary geometries: Haldane sphere and torus shape. On the Haldane sphere, the target state is a unique zero-energy Laughlin ground state, providing a controlled test of the variational workflow and of excited-state reconstruction. On the torus, the problem retains the genuinely two-dimensional periodic character of the quantum Hall liquid and exhibits the threefold topological ground-state degeneracy expected for the $\nu=1/3$ fractional filling factor. This feature makes the torus a more demanding benchmark than the quasi-one-dimensional cylinder or thin-torus limits commonly exploited in state-preparation quantum protocols. We benchmark the hardware-optimized variational states against exact diagonalization using energy estimates, error-mitigated observables, and subspace-containment diagnostics. Our results show that hybrid quantum algorithms can approximately reconstruct the low-energy structure of small fractional quantum Hall systems, including the topological ground-state manifold on the torus. Beyond serving as a benchmark for quantum hardware, this geometry-resolved approach provides a route toward quantum simulations of fractional Chern insulators and strongly correlated topological phases in realistic two-dimensional materials.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();
push @sub_doc_options, '-pdf';

push @file_not_found, '^No file\\s*(.+)\s*$';
add_cus_dep('tex', 'aux', 0, 'makeexternaldocument');

sub makeexternaldocument {
    if ($root_filename ne $_[0]) {
        my ($base_name, $path) = fileparse($_[0]);
        pushd $path;

        my $return = system "latexmk",
                             @sub_doc_options,
                             "-aux-directory=$sub_doc_output",
                             "-output-directory=$sub_doc_output",
                             $base_name;

        if (($sub_doc_output ne '') && ($sub_doc_output ne '.')) {
            rdb_add_generated("$sub_doc_output/$base_name.aux");
            copy "$sub_doc_output/$base_name.aux", ".";
        }

        popd;
        return $return;
    }
}
